Aligning Offline Metrics and Human Judgments of Value for Code Generation Models

Large language models have demonstrated great potential to assist programmers in generating code. For such human-AI pair programming scenarios, we empirically demonstrate that while generated code is most often evaluated in terms of their functional correctness (i.e., whether generations pass available unit tests), correctness does not fully capture (e.g., may underestimate) the productivity gains these models may provide. Through a user study with N = 49 experienced programmers, we show that while correctness captures high-value generations, programmers still rate code that fails unit tests as valuable if it reduces the overall effort needed to complete a coding task. Finally, we propose a hybrid metric that combines functional correctness and syntactic similarity and show that it achieves a 14% stronger correlation with value and can therefore better represent real-world gains when evaluating and comparing models.

==> locks.tex <==
candidate titles:
1. Measuring Alignment Between Offline Metrics and Human Judgments of Value of AI-Pair Programmers?
2. Measuring Alignment Between Metrics and Value of AI-Pair Programmers
3. Measuring Value of AI-Pair Programmers
4. What do people even want from their AI-pair programmers?
3. 





abstract - 
1. intro - 
2. related work - 
3. experiments  - 
4. results - a/b 
        b - 
        c - saleema

5. discussion 

%% terminology/definitions
- Offline metrics: functional correctness and similarity-based metrics
    - pass@1 and pass@k (use \passOne)
        - DO NOT use "accuracy"
    - Normalized Edit Similarity (use \editSim)
        - DO NOT use "edit"
    - Bleu
- Online metrics: programmers'
    - perceived functional correctness (use \perAccuracy)
    - perceived value [in the real world] (use \perValue)
    - perceived effort [required to fix the code] (use \perEffort)
- "programmer" to refer to the person who uses code generation systems
    - DO NOT use "developer"
- "developer" to refer to the person who is developing and deploying code generation systems


%%%%%%%%
    also functional correctness vs accuracy is confusing. we need to choose one. -> I vote correctness :D

    where to use functional correctness vs pass@1? 
    functional correctness vs function testing?
    
    > I think pass@1 for the user study/online is confusing because people always see one generation. 


    cushman - 14 5s
    davinci 1 - 18 5s
    davinci 2 - 15 5s

==> sections/ack.tex <==
\begin{acks}
  authors acknowledge ...
  
\end{acks}
  
% This section has a special environment:
% \begin{verbatim}

% \end{verbatim} 
% Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

==> sections/offline.tex <==
\section{Offline Experiments}
\forough{On terminology: should we use ``functional correctness'' (instead of ``correctness'') and ``similarity metric'' or ``similarity-based metric'' (instead of ``effort'')?}
We ran a series of offline experiments to examine how functional correctness and similarity metrics compare and how they would impact model development and deployment decisions. 

\subsection{How correlated are correctness and effort metrics?}
We first examine correlations between correctness and effort metrics at the level of \textbf{individual generations}. For each scenario of interest (k=1 and k=10), we ran each of our models over each problem in the HumanEval dataset. For k=1, we measure correctness and effort directly on the single generation produced. For k=10, we measure correctness according to section X. 



Next we examine the correlation between correctness and effort at the \textbf{corpus level} over all models we tested. For this we did bootstrapping.... and computed Pearson's correlation. Figures xxx show the results. In all cases, we see strong correlations. 


 


\subsection{How would correctness and effort metrics impact model deployment decisions?}
Studies of AI practitioners show that offline model performance evaluations often gate which models are deployed in the real-world or advanced to further testing with humans-in-the-loop \citet{zhou2022deconstructing}. For these deployment decisions, models are typically run over one or more test datasets and aggregate scores are computed for each model over instances of that dataset for any given metric. Models are then ranked from best to worst according to aggregate metric scores, with the best model being selected for deployment.   

To understand how correctness and effort metrics would impact deployment decisions, we examine how each of our metrics ranks our models according to their average score over the HumanEval dataset. We perform bootstrapping to obtain confidence intervals over average metric scores per model by resampling generations from that model applied to the HumanEval dataset with replacement for 100 samples of size equal to the number of problems in HumanEval (164). Figures \ref{fig:notchplots_at1} and \ref{fig:notchplots_at10} show notched boxplots of average model scores after bootstrapping for both our k=1 and k=10 metrics. From these figures we can see that functional testing (pass@1 and pass@10) would confidently choose davinci-002 over all other models whereas both syntactic similarity metrics less cleanly separate davinci-002 from the next two best models davinci-001 and cushman-001. Functional testing also shows davinci-001 as outperforming cushman-001, whereas similarity metrics flip the ranking of these models at k=1.




\begin{figure*}[t]
  \centering
  \begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/notch_plots_at1.png}
  \captionof{figure}{Offline metric values per model}
  \label{fig:notchplots_at1}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/value_per_model_div_bar.png}
  \captionof{figure}{Online human-judged value per model}
  \label{fig:notchplots_at10}
\end{minipage}
\end{figure*}

% \Bug{G: are the models sorted in any particular order? Would be nice to sort them by size, as opposed to, who created them. Would be nice to very briefly add key observations to the figures.}

\subsection{How would our metrics impact model development decisions?}
While correlations can reveal the strength of the association between metrics (see earlier section), when it comes to understanding their impact on development decisions we instead look at their agreement in terms of partitioning the data into "errors" and "non-errors". [X] showed that most practitioners manually examine individual outputs of NLG systems to help evaluate system performance. While methods for selecting instances to inspect are often ad hoc [], analyzing errors to form hypothesize about how to improve models is recommended [] and has been reported for model evaluation and debugging []. If two metrics agree on where a system is failing, the intuition here is that regardless of what metric is used, practitioners would inspect the same data to determine how to improve the model. For example, [] showed that most practitioners rely on expanding datasets to improve model performance. When error regions are disjoint, different data may be collected to mitigate (e.g., collecting more data for functions with conditions vs those with ....).

\begin{figure*}[t]
  \centering
  \begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/pass_edit_agreement.png}
  \captionof{figure}{Pass vs edit agreement over human-eval data}
  \label{fig:notchplots_at1}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/pass_edit_value_agreement.png}
  \captionof{figure}{Pass vs edit vs value over study data}
  \label{fig:notchplots_at10}
\end{minipage}
\end{figure*}

 

==> sections/online.tex <==
\section{User Study}

\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{0.49\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/notch_plots_at1.png}
  \caption{While Pass@1 suggests that Davinci-2 is a significantly better model, similarity-based metrics find no difference between the top three models.}
  \label{fig:notchplots_at1}
\end{subfigure}%
\hfill
\begin{subfigure}[b]{0.49\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/value_per_model_div_bar.png}
  \caption{Human judgements of perceived value, accuracy, and effort suggest no difference between the top three models. \gagan{Add accuracy and effort to this plot similar to the sub figure a; use same size as a; remove title}
  }
  \label{fig:notchplots_at10}
\end{subfigure}
\caption{Comparison of rankings of five state-of-art code generation models on three offline metrics (a) and three online metrics (b).}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/davinci_value_per_bucket.png}
    \caption{Our user study empirically confirms the scenario in Figure~\ref{fig:??} -- similarity metrics can help identify code suggestions that fail unit tests but are {\em highly} valuable to programmers. The circle indicates such instances for Davinci-2 on the HumanEval.
    % code suggestions that are rated as high value by subjects even when they fail the unit tests.
    \gagan{make the y-axis consistent and circle the second column with high value and tie it with figure 1; decrease width of each column, increase font size.}
    }
    \label{fig:my_label}
\end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/pass_edit_value_corr.png}
         \caption{Both the functional correctness and similarity metric positively correlate with programmer's value -- suggestions that rate high on either offline metric are also rated higher in terms of value. However, functional correctness (left) shows a stronger correlations.\forough{Should we break these into separate figures rather than subfigures? That would allow us to reference specific figures in e.g., 4a.}
         \gagan{fix range of y-axis across hists; }
         }
         \label{fig:y equals x}
     \end{subfigure}
     \hfill

    \begin{subfigure}[b]{0.5\textwidth}
      \centering
          \includegraphics[width=\textwidth]{figures/pass_edit_value_barchart.png}
          \caption{
          Inaccurate but useful code suggestions.
          Left histogram shows suggestions that fail unit but test may be deemed valuable by users. Circle shows a subset of these examples that can be captured by similarity metric plausibly because they are able to reward partial credit to code suggestions.
          % Pass doesn't give partial credit. Edit can when pass fails.
      \label{fig:valuebreakdown}} 
    \end{subfigure}
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/pass_acc_edit_effort.png}
         \caption{
         Perceived accuracy vs perceived effort.
         While pass is more correlated with perceived accuracy, edit is more correlated with perceived effort. \gagan{this figure needs to change. it should be a 2x2 grid. it needs to show that edit correlates more with effort than pass. and pass correlates more with accuracy than edit.}}
         \label{fig:five over x}
     \end{subfigure}
    
    \caption{(a) Correlation between metrics and human value. (b)  Inaccurate but useful code suggestions. (c) Correlation between metrics and perceived accuracy and effort.}
    \label{fig:three graphs}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/pass_edit_value_agreement_2.png}
    \caption{Distribution of errors (i.e., low performing generations) as judged by two offline metrics (pass@1 \& edit) and 
    the online metric of human perceived value. Error analysis along a given metric can help developers design interventions to improve models (e.g., by gathering more training data on errors), but 
    we observed that while these two offline metrics may not agree on errors but together they may better capture errors that truly matter -- lowest overall value for users.
    \gagan{Do we really need to present all 5 models together? Why don't we focus on the top 2 or 1? Otherwise this figure is pretty overwhelming.}}
    \label{fig:agreement}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/value_per_model.png}
    \caption{Distribution of participant perception of value of code suggestions (Likert scale) for five state-of-the-art code generation models. The survey asked {\em Assuming you were a programmer writing a solution to the task, and you received snippet A ... how useful will this be to you?} 
    \gagan{Fix size convert into box plot and make it similar to the box plot figure from the offline experiments. Saleema: Box plots aren't advised for ordinal data. The closest thing to get a similar shape for comparison is a diverging bar chart. I tried this in Fig 9. Let's discuss.}
    }
    \label{fig:my_label}
\end{figure*}

\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/notch_plots_at1.png}
  \caption{Offline metric values per model}
  \label{fig:notchplots_at1}
\end{subfigure}%
\hfill
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/value_per_model_div_bar.png}
  \caption{Online human-judged value per model \gagan{No reason for this fig to be this wide.}}
  \label{fig:notchplots_at10}
\end{subfigure}
\caption{}
\end{figure*}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/davinci_value_per_bucket.png}
    \caption{Suggestions are rated as high value even when they dont pass the unit test \gagan{make the y-axis consistent and circle the second column with high value and tie it with figure 1}}
    \label{fig:my_label}
\end{figure}


 
\begin{figure}
    \centering
    \includegraphics[width=0.3\linewidth]{figures/metrics-correlation.png}
    \caption{correlation between metrics and different dimensions of human preferences}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.3\linewidth]{figures/placeholder}
    \caption{Scatter plot showing correlation between edit score and perceived effort for inidividual generations.}
    \label{fig:my_label}
\end{figure}





\begin{figure*}[!t]
  \centering
  \includegraphics[width=\textwidth]{figures/studyheader.pdf}
  \caption{(a) Screenshot of a section in the main study task. For each task, participants were shown a pair of code snippets and asked to provide ratings on a likert type scale for 3 questions corresponding to accuracy (framed as program equivalence),  value of generated code and effort. 
  \label{fig:studyheader}} 
\end{figure*}
 

\subsection{Study Results}
We conducted an analysis of developers' judgements of the value of generated code. In cases where the generations pass their respective offline unit tests, developer assigned value is high, with both a median and mode of 5 (the maximum value of the scale). Conversely, when generations fail their unit tests, value is judged to be low, with a median of 2 and a mode of 1 (the lowest value on the scale). These differences are highly statistically significant by the  Mann–Whitney U test ($p < 0.001$).

The above pattern (median 5 vs. 2, mode 5 vs. 1), is mirrored when the analysis is repeated for judgments of both effort and correctness. This is not surprising given that both correlate with value, with correctness showing a stronger tendency in this regard ($r=0.94$; $p < .001$ vs $r=0.87$; $p < .001$). 

Similarly, we compute the correlation between the normalized edit similarity metric and judgments of value, and find positive correlation ($r=0.48$, $p < .001$). The similarity metric is similarly positively correlated with correctness (\adam{TODO: fill in}), and effort (\adam{TODO: fill in})


\ignore{
\textbf{Do perceived correctness and perceived effort correlate with what developers value online?}
We conducted an analysis of the correlation between developers' judgements of the value of generated code and their perceived correctness of the code and amount of effort it would take to fix the generated code. We find that both perceived correctness and perceived effort correlate with what developers value, and perceived effort shows a stronger correlation ($r=0.94$, $p < .001$) than perceived correctness with value ($r=0.87$, $p < .001$).

We were interested in understanding how human perception on the functional behaviour of code (if code is equivalent ... as an indirect measure of accuracy), perception of effort required to fix the code if any are related to perceptions on the value of generated code. We find that both indicators (accuracy, effort) are correlated with themselves and also correlated with value. This is indicated of a user value being a formative construct jointly expressed by both indicators. Interestingly, we find that the correlation between effort and value (pearson coeff=0.94, p=0.000) is stronger than the correlation between accuracy and value (pearson coeff=0.87, p=0.000). 
}
